Data-driven emergence of convolutional structure in neural networks

Exploiting data invariances is crucial for efficient learning in both artificial and biological neural circuits. Understanding how neural networks can discover appropriate representations capable of harnessing the underlying symmetries of their inputs is thus crucial in machine learning and neuroscience. Convolutional neural networks, for example, were designed to exploit translation symmetry and their capabilities triggered the first wave of deep learning successes. However, learning convolutions directly from translation-invariant data with a fully-connected network has so far proven elusive. Here, we show how initially fully-connected neural networks solving a discrimination task can learn a convolutional structure directly from their inputs, resulting in localised, space-tiling receptive fields. These receptive fields match the filters of a convolutional network trained on the same task. By carefully designing data models for the visual scene, we show that the emergence of this pattern is triggered by the non-Gaussian, higher-order local structure of the inputs, which has long been recognised as the hallmark of natural images. We provide an analytical and numerical characterisation of the pattern-formation mechanism responsible for this phenomenon in a simple model and find an unexpected link between receptive field formation and tensor decomposition of higher-order input correlations. These results provide a new perspective on the development of low-level feature detectors in various sensory modalities, and pave the way for studying the impact of higher-order statistics on learning in neural networks.

==> contents/odes.tex <==
\section{Dynamics of one-pass stochastic gradient descent}
What follows is a brief review of the main steps in the derivation of the update
equations for the order parameters. For a general introduction, we refer the
reader to the classic works \cite{SaadSollaExact, SaadSollaOnline}. We follow
closely the analysis of \citet{refinetti2021classifying}.

\subsection{Joint Gaussian for pre-activations}

Calling $\lambda_{k}^{\mu}=\sum_{i}w_{ki}x_{i}^{\mu}$, the average
pre-activation of hidden unit $k$ is $\left\langle h_{k}^{\mu}\right\rangle =\lambda_{k}+b_{k}$
and the covariances of bias-removed pre-activations reads:

\[
q_{kl}^{\mu}\equiv\left\langle \lambda_{k}^{\mu}\lambda_{l}^{\mu}\right\rangle =\sum_{ij}w_{ki}w_{lj}\left\langle x_{i}^{\mu}x_{i}^{\mu}\right\rangle =WC^{\mu}W^{T}=\tilde{W}\Lambda^{\mu}\tilde{W}^{\dagger}
\]
where we diagonalized the covariance matrices in the Fuorier Basis
$F$ by $C^{\mu}=F\Lambda^{\mu}F^{\dagger}$ and $\tilde{w}_{k\tau}=\sum_{i}F_{i\tau}w_{ki}$
the discrete Fourier Transform of the weight vector $\boldsymbol{w}_{k\cdot}$.

\subsection{Loss}

The mean-squared loss reads:
\[
L=\frac{1}{2M}\sum_{\mu=1}^{M}\left(\sum_{k}v_{k}g\left(h_{k}^{\mu}\right)-y^{\mu}\right)^{2}+\frac{\gamma}{2}\sum_{ki}w_{ki}^{2}
\]
Averaging over the input data, the loss can be written solely in terms
of the order paramters $q^{\mu}$'s:

\subsection{Average gradient}

When an input $x^{\mu}$ is presented, the gradient updates for the
are:
\begin{align*}
 & \Delta b_{k}^{\mu}=\frac{\eta}{D}\delta_{k}^{\mu}\\
 & \Delta w_{ki}^{\mu}=\frac{\eta}{\sqrt{D}}\delta_{k}^{\mu}x_{i}^{\mu}-\frac{\eta\gamma}{\sqrt{D}}w_{ki}\\
 & \Delta v_{k}^{\mu}=\frac{\eta}{D}\left(y^{\mu}-\sum_{l}v_{l}g\left(h_{l}^{\mu}\right)\right)g\left(h_{k}^{\mu}\right)
\end{align*}
where we called $\delta_{k}^{\mu}\equiv-\frac{\partial L^{\mu}}{\partial h_{k}^{\mu}}=v_{k}\left(y^{\mu}-\sum_{l}v_{l}g\left(h_{l}^{\mu}\right)\right)g^{'}\left(h_{k}^{\mu}\right)$
and employed the a scaling of the update coefficients: $\frac{\eta_{w}}{\sqrt{D}}$,$\frac{\eta_{v}}{D}$,
$\frac{\eta_{b}}{D}$. We will now proceed to average Eqs with respect
to the input data $x^{\mu}$'s. A critical ingredient in the ensuing
derivation is the computation of non-linear moments for weakly correlated
variables as linear functions of their covariances, using a Taylor
expantion of the probability density function. We employ results obtained
in \cite{GoldtModeling} for centered variables and soon generalized to the
general case~\cite{refinetti2021classifying}. We rewrite here their results for two and three variables:

\paragraph*{Update of second-layer weights and bias}
Averaging Eqs over the input data one gets
\begin{align*}
\frac{\Delta v_{k}}{\Delta t}= & \frac{\eta_{v}}{P}\sum_{\mu}\left(y^{\mu}\left\langle g\left(h_{k}^{\mu}\right)\right\rangle -\sum_{l}v_{l}\left\langle g\left(h_{k}^{\mu}\right)g\left(h_{l}^{\mu}\right)\right\rangle \right)\\
\frac{\Delta b_{k}}{\Delta t}= & \frac{\eta_{b}}{P}v_{k}\sum_{\mu}\left(y^{\mu}\left\langle g^{'}\left(h_{k}^{\mu}\right)\right\rangle _{\mu}-\sum_{l}v_{l}\left\langle g^{'}\left(h_{k}^{\mu}\right)g\left(h_{l}^{\mu}\right)\right\rangle _{\mu}\right)
\end{align*}


\paragraph*{Update of first-layer weights}

Rotating Eq in Fourier space and averaging over the input in the $\mu$th
class, we get:
\begin{align*}
\left\langle \Delta w_{k\tau}^{\mu}\right\rangle _{\mu} & =\left\langle \frac{\eta}{\sqrt{D}}v_{k}\left(y^{\mu}-\sum_{l}v_{l}g\left(h_{k}^{\mu}\right)\right)g^{'}\left(h_{k}^{\mu}\right)\tilde{x}_{\tau}^{\mu}\right\rangle _{\mu}-\frac{\eta\gamma}{D}\tilde{w}_{k\tau}=\\
 & \frac{\eta}{\sqrt{D}}y^{\mu}v_{k}\left\langle g^{'}\left(h_{k}^{\mu}\right)\tilde{x}_{\tau}^{\mu}\right\rangle _{\mu}-\frac{\eta}{\sqrt{D}}v_{k}\sum_{l}v_{l}\left\langle g^{'}\left(h_{k}^{\mu}\right)g\left(h_{l}^{\mu}\right)\tilde{x}_{\tau}^{\mu}\right\rangle _{\mu}-\frac{\eta\gamma}{D}\tilde{w}_{k\tau}
\end{align*}
Now, since $\tilde{x}_{\tau}^{\mu}=\sum_{i}F_{i\tau}x_{i}^{\mu}$
and $F$ diagonalizes each $C^{\mu}$'s: 
\[
\left\langle \lambda_{k}^{\mu}\tilde{x}_{\tau}^{\mu}\right\rangle =\frac{1}{\sqrt{D}}\tilde{w}_{k\tau}\rho_{\tau}^{\mu}
\]
Using Eq CITE we get:
\[
\left\langle g^{'}\left(h_{k}^{\mu}\right)\tilde{\xi}_{\tau}^{\mu}\right\rangle _{\mu}=\frac{1}{\sqrt{D}}\frac{\tilde{w}_{k\tau}\rho_{\tau}^{\mu}}{q_{kk}}\left\langle g'\left(h_{k}^{\mu}\right)\lambda_{k}^{\mu}\right\rangle _{\mu}
\]
For the term involving three jointly Gaussin distributed variables, we use Eqs CITE to obtain, for $k\neq l$:
\begin{align}
\left\langle g^{'}\left(h_{k}^{\mu}\right)g\left(h_{l}^{\mu}\right)\tilde{x}_{\tau}^{\mu}\right\rangle _{\mu}&=\frac{\rho_{\tau}^{\mu}}{\sqrt{D}}\frac{1}{q_{kk}q_{ll}-q_{kl}^{2}}\left[\left(q_{ll}\tilde{w}_{k\tau}-q_{kl}\tilde{w}_{l\tau}\right)\left\langle g^{'}\left(h_{k}^{\mu}\right)\lambda_{k}^{\mu}g\left(h_{l}^{\mu}\right)\right\rangle +\right.\nonumber\\&\left.\left(q_{kk}\tilde{w}_{l\tau}-q_{kl}\tilde{w}_{k\tau}\right)\left\langle g^{'}\left(h_{k}^{\mu}\right)\lambda_{l}^{\mu}g\left(h_{l}^{\mu}\right)\right\rangle \right]
\end{align}
and for $k=l$:
\[
\left\langle g^{'}\left(h_{k}^{\mu}\right)g\left(h_{k}^{\mu}\right)\tilde{x}_{\tau}^{\mu}\right\rangle _{\mu}=\frac{1}{\sqrt{D}}\frac{\tilde{w}_{k\tau}\rho_{\tau}^{\mu}}{q_{kk}}\left\langle g'\left(h_{k}^{\mu}\right)\lambda_{k}^{\mu}g\left(h_{k}^{\mu}\right)\right\rangle _{\mu}
\]

\subsection{Order parameter updates}

Multiplying and using the definition $Q_{kl}^{\mu}=\frac{1}{D}\sum_{\tau}\tilde{w}_{k\tau}\tilde{w}_{l\tau}^{*}\rho_{\tau}^{\mu}$,
we get to an update equation for $q^{\mu}$ in closed form
\[
\Delta q_{kl}^{\mu}=\frac{1}{D}\sum_{\tau}\rho_{\tau}^{\mu}\left[\sum_{\nu}\left(\Delta\tilde{w}_{k\tau}^{\nu}\tilde{w}_{l\tau}+\tilde{w}_{k\tau}\Delta\tilde{w}_{l\tau}^{\nu}\right)+\sum_{\nu}\Delta\tilde{w}_{k\tau}^{\nu}\Delta\tilde{w}_{l\tau}^{\nu}\right]
\]
The linear terms in $\Delta\tilde{w}$ 
\begin{align*}
\delta q_{kl}^{\mu,\left(1\right)}=\Delta\tilde{w}_{k\tau}^{\mu}\tilde{w}_{l\tau}+\tilde{w}_{k\tau}\Delta\tilde{w}_{l\tau}^{\mu}= & \frac{\eta}{D}\sum_{\tau}m_{l\tau}^{\nu}v_{k}\left(y^{\nu}\left\langle g^{'}\left(h_{k}^{\nu}\right)\right\rangle _{\nu}-\sum_{n}v_{n}\left\langle g^{'}\left(h_{k}^{\nu}\right)g\left(h_{n}^{\nu}\right)\right\rangle _{\nu}\right)+\\
 & \frac{\eta}{D}\sum_{\tau}y^{\nu}v_{k}\rho_{\tau}^{\nu}\frac{\tilde{w}_{k\tau}\tilde{w}_{l\tau}^{*}}{Q_{kk}^{\nu}}\left\langle g'\left(h_{k}^{\nu}\right)\lambda_{k}^{\nu}\right\rangle _{\nu}\\
 & -\frac{\eta}{D}\sum_{\tau}v_{k}^{2}\frac{\tilde{w}_{k\tau}\tilde{w}_{l\tau}^{*}\rho_{\tau}^{\nu}}{Q_{kk}^{\nu}}\left\langle g'\left(h_{k}^{\nu}\right)\lambda_{k}^{\nu}g\left(h_{k}^{\nu}\right)\right\rangle _{\nu}\\
 & -\frac{\eta}{D}\sum_{\tau}\sum_{m\neq k}\frac{v_{k}v_{m}\rho_{\tau}^{\nu}}{Q_{kk}^{\nu}Q_{mm}^{\nu}-\left(Q_{km}^{\nu}\right)^{2}}\left[\left(Q_{mm}^{\nu}\tilde{w}_{k\tau}\tilde{w}_{l\tau}^{*}-Q_{km}^{\nu}\tilde{w}_{m\tau}\tilde{w}_{l\tau}^{*}\right)\left\langle g^{'}\left(h_{k}^{\nu}\right)\lambda_{k}^{\nu}g\left(h_{m}^{\nu}\right)\right\rangle \right.\\
 & \left.+\left(Q_{kk}^{\nu}\tilde{w}_{m\tau}\tilde{w}_{l\tau}^{*}-Q_{km}^{\nu}\tilde{w}_{m\tau}\tilde{w}_{l\tau}^{*}\right)\left\langle g^{'}\left(h_{k}^{\nu}\right)\lambda_{m}^{\nu}g\left(h_{m}^{\nu}\right)\right\rangle \right]\\
 & -\frac{\eta\gamma}{D}\sum_{\tau}\tilde{w}_{k\tau}\tilde{w}_{l\tau}^{*}+
\end{align*}
where we again made extensive use of Eqs to express the gaussian averages
as linear functions of the $\rho_{\tau}^{\mu}$ eigenvalues pre-activation
covariances. The quadratic term $\delta q_{kl}^{\mu,\left(2\right)}$
contains terms of the form:
\[
\frac{1}{D}\sum_{\tau\nu}\rho_{\tau}^{\mu}\left\langle g^{'}\left(h_{k}^{\nu}\right)g^{'}\left(h_{k}^{\nu}\right)g\left(h_{n}^{\nu}\right)g\left(h_{m}^{\nu}\right)\left(\tilde{\xi}_{\tau}^{\nu}\tilde{\xi}_{\tau}^{\sigma}\right)\right\rangle _{\nu}\sim\sum_{\nu}\left(\frac{1}{D}\sum_{\tau}\rho_{\tau}^{\mu}\left\langle \tilde{\xi}_{\tau}^{\nu}\tilde{\xi}_{\tau}^{\sigma}\right\rangle _{\nu,\sigma}\right)\left\langle g^{'}\left(h_{k}^{\nu}\right)g^{'}\left(h_{k}^{\nu}\right)g\left(h_{n}^{\nu}\right)g\left(h_{m}^{\nu}\right)\right\rangle _{\nu}
\]
Now, since $\left\langle \tilde{\xi}_{\tau}^{\nu}\tilde{\xi}_{\tau}^{\sigma}\right\rangle =\delta_{\nu\sigma}\rho_{\tau}^{\nu}$,
we set $\chi^{\mu}=\frac{1}{D}\sum_{\tau}\rho_{\tau}^{\mu}\left\langle \left(\tilde{\xi}_{\tau}^{\nu}\right)^{2}\right\rangle _{\nu}=\frac{1}{D}\sum_{\tau}\left(\rho_{\tau}^{\mu}\right)^{2}$.

\subsection{Explicit expressions for Gaussian integrals involing the erf fuctions}
Gaussian integrals involving centered multinomial Gaussian and the $g$ function have been previously reported in the online learning literature \cite{SaadSollaExact,BiehlLearning,GoldtDynamics}. The generalization to non-centered Gaussian densities is straightforward in most cases. Integrals involving more than one $g$ term or a combination of linear and $g$ terms can be calculated by recursive quadratic completion and repeated application of the following identities, easily derived from notable Gaussian identities \cite{OwenTable,NgTable}:
\begin{align}
\frac{1}{\sqrt{2\pi}}\int g\left(x\right)e^{-\frac{1}{2}\left(ax+b\right)^{2}}dx=&-\frac{1}{a}g\left(\frac{b}{\sqrt{a^{2}+1}}\right)\\
\frac{1}{\sqrt{2\pi}}\int dxg^{2}\left(a+bx\right)e^{-\frac{x^{2}}{2}}=&1-8T\left(\frac{a}{\sqrt{1+b^{2}}},\frac{1}{\sqrt{1+2b^{2}}}\right)\\
I_{gg}\left(a,b;c,d\right)\equiv\frac{1}{\sqrt{2\pi}}\int dxg\left(a+bx\right)g\left(c+dx\right)e^{-\frac{x^{2}}{2}}=&1-4\left[T\left(\frac{a}{\sqrt{1+b^{2}}},\frac{c+cb^{2}-abd}{a\sqrt{1+b^{2}+d^{2}}}\right)\right. \nonumber \\
&\left.+T\left(\frac{c}{\sqrt{1+d^{2}}},\frac{a+ad^{2}-bcd}{c\sqrt{1+b^{2}+d^{2}}}\right)\right. \nonumber \\
&\left.+\begin{cases}
0 & ac>0\qquad\text{or}\qquad ac=0,\;c\;\text{or}\;a<0\\
\frac{1}{2} & ac>0\qquad\text{or}\qquad ac=0,\;c\;\text{or}\;a<0
\end{cases}\right]
\end{align}
where $T$ is the Owen's $T$ function \cite{OwenTable}, defined as
\begin{equation}
T\left(h,a\right)=\frac{1}{2\pi}\int_{0}^{a}\frac{e^{-\frac{x^{2}}{2}\left(1+h^{2}\right)}}{1+x^{2}}    
\end{equation}
We report our results in the following. The symbol $\Delta_{i_{1}i_{2},\ldots,i_{n}}$
stands for the $i_{1},i_{2},\ldots,i_{n}$ sub-determinant of the
covariance matrix
\[
\Delta_{i_{1}i_{2},\ldots,i_{n}}=\left|\begin{array}{cccc}
q_{i_{1}i_{1}} & q_{i_{1}i_{2}} & \dots & q_{i_{1}i_{n}}\\
\dots & q_{i_{2}i_{2}} & \dots & q_{i_{2}i_{n}}\\
\dots & \dots & \dots & \dots\\
\dots & \dots & \dots & q_{i_{n}i_{n}}
\end{array}\right|\text{.}
\]
\begin{equation}
\left\langle g\left(x+a\right)g\left(y+b\right)\right\rangle =-I_{gg}\left(\sqrt{q_{22}},b;-\frac{q_{12}}{\sqrt{q_{22}+\Delta_{12}}},-\frac{a\sqrt{q_{22}}}{\sqrt{q_{22}+\Delta_{12}}}\right)
\end{equation}
\begin{equation}
\left\langle g^{'}\left(x+a\right)yg\left(z+c\right)\right\rangle =\sqrt{\frac{2}{\pi\left(1+q_{11}\right)}}e^{-\frac{a^{2}}{2\left(1+q_{11}\right)}}\left[\sqrt{\frac{2}{\pi}}\Omega e^{-\frac{\Theta^{2}}{2}}+\frac{aq_{12}}{1+q_{22}}g\left(-\Theta\right)\right]
\end{equation}
where
\begin{align}
\Theta= & \frac{c\left(1+q_{11}\right)-aq_{13}}{\sqrt{1+q_{11}}\sqrt{1+q_{11}+q_{33}+D_{13}}}\\
\Omega= & \frac{q_{23}\left(1+q11\right)-q_{12}q_{13}}{\sqrt{1+q_{11}}\sqrt{1+q_{11}+q_{33}+D_{13}}}
\end{align}

\begin{equation}
\left\langle g^{'}\left(h_{1}\right)g^{'}\left(h_{2}\right)g\left(h_{3}\right)g\left(h_{4}\right)\right\rangle =-\frac{2}{\pi}\frac{e^{-\frac{\Theta}{2}}}{\sqrt{D}_{0}}I_{4}^{2}\left(d-\frac{\nu_{1}}{D_{0}},\sqrt{\frac{D_{1}}{D_{0}}};\frac{\nu_{2}}{D_{0}\sqrt{\left(D_{1}+D_{2}\right)D_{1}}},\frac{\nu_{3}}{\sqrt{\left(D_{1}+D_{2}\right)D_{0}}}\right)
\end{equation}
where
\begin{align}
\Theta= & \frac{b^{2}\left(1+q_{11}\right)+a^{2}\left(1+q_{22}\right)-2abq_{12}}{D_{0}}\\
D_{0}= & 1+q_{11}+q_{22}+\Delta_{12}\\
D_{1}= & q_{44}+\Delta_{124}+\Delta_{14}+\Delta_{24}\\
D_{2}= & \Delta_{134}+\Delta_{234}+\Delta_{34}+D_{0}\\
\nu_{1}= & \frac{b\left(\left(1+q_{11}\right)-q_{12}q_{14}\right)+a\left(\left(1+q_{11}\right)q_{14}-q_{12}q_{24}\right)}{D_{1}}\\
\nu_{2}= & \left(bq_{12}q_{13}-aq_{13}\left(1+q_{22}\right)+c\left(1+q_{11}-q_{12}^{2}+q_{22}+q_{11}q_{22}\right)-b\left(1+q_{11}\right)q_{23}+aq_{12}q_{23}\right)\\
 & \left(q_{14}^{2}\left(1+q_{22}\right)-2q_{12}q_{14}q_{24}+\left(1+q_{11}\right)q_{24}^{2}-\left(1+q_{11}-q_{12}^{2}+q_{22}+q_{11}q_{22}\right)q_{44}\right)\\
\nu_{3}= & -q_{12}q_{14}q_{23}+q_{13}\left(q_{14}+q_{14}q_{22}-q_{12}q_{24}\right)+q_{12}^{2}q_{34}+\left(1+q_{11}\right)\left(q_{23}q_{24}-\left(1+q_{22}\right)q_{34}\right)
\end{align}


==> contents/significance.tex <==
The interplay between data symmetries and network architecture is key for efficient learning in neural networks. Convolutional neural networks perform well in image recognition by exploiting the translation invariance of images. However, learning convolutional structure directly from data has proven elusive. Here we show how a neural network trained on translation-invariant data can autonomously develop a convolutional structure. Our work thus shows that neural networks can learn representations that exploit the data symmetries autonomously, by exploiting higher-order data statistics. We finally identify the maximisation of non-Gaussianity as a guiding principle for representation learning in our model, linking discriminative vision tasks and unsupervised feature extraction.
